Version Reconciliation for Collaborative Databases

We propose MindPalace, a prototype of a versioned database for efficient collaborative data management. MindPalace supports offline collaboration, where users work independently without real-time correspondence. The core of MindPalace is a critical step of offline collaboration: reconciling divergent branches made by simultaneous data manipulation. We formalize the concept of auto-mergeability, a condition under which branches may be reconciled without human intervention, and propose an efficient framework for determining whether two branches are auto-mergeable and identifying particular records for manual reconciliation.

==> acmart-preload-hook.tex <==
\PassOptionsToPackage{dvipsnames}{xcolor}
